DeepSpline: Data-Driven Reconstruction of Parametric Curves and Surfaces

Reconstruction of geometry based on different input modes, such as images or point clouds, has been instrumental in the development of computer aided design and computer graphics. Optimal implementations of these applications have traditionally involved the use of spline-based representations at their core. Most such methods attempt to solve optimization problems that minimize an output-target mismatch. However, these optimization techniques require an initialization that is close enough, as they are local methods by nature. We propose a deep learning architecture that adapts to perform spline fitting tasks accordingly, providing complementary results to the aforementioned traditional methods. We showcase the performance of our approach, by reconstructing spline curves and surfaces based on input images or point clouds.

==> source/from_research_proposal.tex <==
\section{Differentiable Modeler}
\paragraph{Primitives and Splines}
As vital representations of geometric designs, primitives of curves, surfaces, and volumes are the most elementary building blocks of modern design systems.
In industrial designs, most of the representations are splines, due to their simplicity for manipulation, local support, sparse representation, and flexibility regarding smoothness and sharpness.
Many classic works in the traditional Computer Aided Geometric Design community strived to improve such representations from different aspects in the past decades.
Recently, there is a family of work in inverse modeling that targets to create spline curves or spline patches with given data, including my work~\cite{dev16}, where one of the problems solved is to approximate point clouds by developable surfaces.


\paragraph{Expressiveness and Differentiability}
With the advancement of reinforcement learning and deep learning, the intriguing question is that how can we leverage both the geometric modeling capability of the standard geometric algorithm and the powerfulness of machine learning algorithms.
To achieve both, it is important that the core building blocks could be sufficient to convey the design ideas of individual designers and utilized by machine learning algorithms at the same time.
The first aspect requires sufficient expressiveness of the modeler.
The second perspective demands that the modeler should be differentiable to provide adequate feedback for a learning algorithm.
There are two ways to achieve such a balance between expressiveness and differentiability. 
One straightforward way is to wrap the optimization based tools to have an interface to provide gradient to be used by machine learning approaches.
However, a more appealing alternative is to completely replace inverse modeling procedure by learning based approaches, in a way similar to the PointNet~\cite{qi2016pointnet}.
In other words, can we devise a modeler that could generate spline- or subdivision-based curves and surface conditioned on given data of varied forms, e.g., point clouds, signed distance fields, or semantic information?
This problem could be studied individually in 2D and 3D, with an exploratory study carried on 2D first before delving into 3D.

% Oriented boxes had been extensively used in learning simply regarded as proxies of geometric shapes.
% Many of the following procedure to assemble the shapes are based on filling the volume with the voxels or deforming existing shapes.

% Connections to previous work: design with constraints. The implicit function representation also shares similarities with the GRASS idea: the shapes does have both dimensions and codimensions. A lot of generative models explores the subspace with the same dimension as the , while the fact is that the.

% TODO: The previous papers; The interface of the FreeCAD library.


\begin{figure}[b]
	\includegraphics[width=0.4\columnwidth]{images/spline_fitting}
	\hfill
	\begin{minipage}[b]{.58\columnwidth}
	\caption{
\label{fig:spline_fitting}
Fitting a point cloud by a spline curve by minimizing a distance measure between the spline curve and the point cloud works well locally with a given good initialization~\protect\cite{wang2006fitting}.
However, a major challenge is to find the initialization of the control points, especially if the curve has self-intersections.
}
\end{minipage}
\end{figure}

\subsection{2D}
\paragraph{Reconstructing Lines and Curves on Plane}
As a small example to have some concrete and actionable items, we plan to start with the simplest 2D geometric elements and curves tentatively together with Lin Shao, Jiahui Huang, and Olga Diamanti.
The forms of the input include both point clouds and pixelized or voxelized data.
All the problems would be trained on synthetic data, either a set of points on a plane or raster images generated based on vector graphics.
The following lists a set of geometric primitive in 2D and the parameters we would like to recover:

\begin{itemize}
    \item Straight line segments: two ends of a line segment.
    \item Arcs: the circle center and the arc parameter range.
    \item Polyline: the sequence of vertices.
    \item Spline curves: the sequence of control points.
\end{itemize}

Most of the problems have the implication that the neural network should learn how to solve a least-squares fitting problem with given data provided as images.
Two fundamental questions arise naturally: 1) how to devise a learning architecture to recover the 2D primitives, and 2) how to design the loss function of the predicted fitting.
The second one is particularly interesting to me as there are multiple alternatives of different geometric nature connected to traditional CAGD problems.
In general, the loss function measures the difference between a ground truth curve and a predicted curve.
Here, the differences between two curves could be measured in different ways, such as point to point distances, differences between the normal vectors.
In optimization based approaches such as~\cite{wang2006fitting}, it is discovered that the normal information leads to much faster convergence.
Therefore, a particular idea we would like to try is how the information of normal vectors and fields could help the convergence of approximation and learning.

\subsection{3D}
\paragraph{Reconstructing Surfaces and Volumes}
Similar to the case in 2D, the 3D surfaces can also be represented by different primitives.
The following are some of the basic primitives and their corresponding parameters that we are interested:

\begin{itemize}
    \item Ellipsoid: the scaling factors and orientation.
    \item Cuboids: the center, size, and orientation.
    \item Spline or subdivision surfaces: control points.
\end{itemize}

Similar to the case in 2D, a particular question I aim to answer is if and how the proximity of normals, or a Sobolev metric, could help the convergence of the learning process.
Another challenge which is shared by spline curves and spline surfaces is how many control points and which degree shall we choose.
For this problem, a possible way is to start from a large number of initial control points and give a parsimonious reward to the agent when a control point is removed.
A common misconception about splines and spline surfaces is that they are more suitable to represent curves and surfaces that are smooth than those with sharp corners or boundaries.
In fact, by coinciding control points a smooth intersect can degenerate to a sharp corner naturally.
However, how splines could handle both sharp and smooth corners and borders in the context of learning environment is a question by itself that needs be studied.

\begin{figure}[tb]
  \includegraphics[width=\columnwidth]{images/approx}
  \caption{
    Approximating point clouds by developable patches through optimization.
    It has a similar challenge as in the 2D case.
}
\label{fig:approx}
\end{figure}

\paragraph{Possible Advantages of Learning}
As a major difficulty for optimization based methods is how to find the proper initialization of the control points.
However, overviewing the global energy landscape is a possible advantage of learning based approaches.
Compared with a method purely based on optimization, it is speculated that an approach based on machine learning may not need initialization.
Moreover, it is hoped that it will be more robust with respect to self-intersections, for both curves and surfaces, due to the nonlinear nature of hidden layers.


